ASMA-Tune: Unlocking LLMs' Assembly Code Comprehension via Structural-Semantic Instruction Tuning

Assembly code analysis and comprehension play critical roles in applications like reverse engineering, yet they face substantial challenges due to low information density and a lack of explicit syntactic structures. While traditional masked language modeling (MLM) approaches do not explicitly focus on natural language interaction, emerging decoder-focused large language models (LLMs) demonstrate partial success in binary analysis yet remain underexplored for holistic comprehension. We present Assembly Augmented Tuning, an end-to-end structural-semantic instruction tuning framework that synergizes encoder architecture with decoder-based LLMs through a projector module, where the assembly encoder extracts hardware-level structural features, the projector bridges representations with the semantic space, and the instruction-tuned LLM preserves natural language capabilities. Experimental results demonstrate three key advantages: (1) State-of-the-art performance in assembly comprehension with +39.7% Recall@1 and +17.8% MRR improvements over GPT-4-Turbo, (2) Consistent enhancements across base models (24.6-107.4% Recall@1 and 15.2-106.3% MRR on Qwen2.5-Coder, Deepseek-Coder and CodeLlama variants), and (3) Superior instruction-following capabilities (41.5%-118% improvements) with controlled code generation degradation (-8.9% to -35% across architectures).

==> tables/Ablation-BCSD.tex <==
% \begin{table}[]
%     \centering
%     \scriptsize
%     \begin{tabular}{@{}l|ll@{}}
%         \toprule
%         Assembly features     & Before & After \\ \midrule
%         Full training         &        &       \\
%         No Pre-training       &        &       \\
%         No Funetuning         &        &       \\
%         7B model size         &        &       \\ \bottomrule
%     \end{tabular}
%     \caption{Ablation Study on BCSD Task}
%     \label{tab:ablation2}
% \end{table}

==> tables/Ablation_ASMABench.tex <==
% \begin{table}[t]
%     \centering
%     \scriptsize
%     \begin{tabular}{@{}l|llll@{}}
%         & Conversation & Detail description & Complex reasoning & All \\ \midrule
%         Full data                      &              &                    &                   &     \\
%         \textit{No Detail description} &              &                    &                   &     \\
%         \textit{No Conversation}       &              &                    &                   &     \\
%         \textit{No Complex Reasoning}  &              &                    &                   &     \\
%         \textit{No Instruction Tuning} &              &                    &                   &     \\ \bottomrule
%     \end{tabular}
%     \caption{Ablation Study on ASMA-Bench(BinaryCrop)}
%     \label{tab:ablation1}
% \end{table}

==> tables/Human-model-Assessment.tex <==
% \begin{table}[h]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|llll@{}}
% \toprule
%                       & Conversation & Detail description & Complex reasoning & All \\ \midrule
% Human                 &              &                    &                   &     \\
% GPT-4-Turbo             &              &                    &                   &     \\
% \bottomrule
% \end{tabular}%
% }
% \caption{}
% \label{table5:Human and model Assessment}
% \end{table}

==> tables/datasets_detail.tex <==
\begin{table}[h]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt} % 增加列间距
\renewcommand{\arraystretch}{1.5} % 增加行高
\begin{tabular}{ccc}
\toprule
Project Name  & Functions & Proportion\\ \midrule
Binutils     & 24001            & 56\%       \\
Coreutils    & 1152            & 3\%        \\
Curl         & 666            & 2\%        \\
ImageMagick  & 1422              & 3\%        \\
SQLite       & 1632              & 4\%        \\
OpenSSL      & 5302            & 12\%       \\
Putty        & 8809           & 20\%       \\ \bottomrule

\end{tabular}
\caption{Details of datasets.}
\label{tab:detail_datasets}
%\vspace{-2mm}
\end{table}


==> tables/eval-ASMABench_old.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt} % 增加列间距
\renewcommand{\arraystretch}{1.5} % 增加行高
%\vspace{-2mm}
\begin{tabular}{r|cccc}
\toprule
\multicolumn{1}{c|}{\textbf{Models}}                & Conversation & Detail description & Complex reasoning & All    \\ \midrule
GPT-4-Turbo     & 82.65     & 85.42             & 87.20     & 85.09 \\
Qwen2.5-Coder-Instruct-GGUF\textsubscript{14B}     & 81.67        & 63.60               & 76.63             & 73.97 \\
CodeLlama-Instruct\textsubscript{13B}              & 48.62        & 33.88              & 52.73             & 45.08 \\
DeepSeek-Coder-V2-Lite-Instruct\textsubscript{16B} & 74.98        & 67.47              & 69.40              & 70.62 \\
ASMA-Tune\textsubscript{13B}(Ours) & \cellcolor[HTML]{EFEFEF}90.10 & \cellcolor[HTML]{EFEFEF}85.15 & \cellcolor[HTML]{EFEFEF}86.12 & \cellcolor[HTML]{EFEFEF}87.12 \\ \bottomrule
\end{tabular}%
%For a given set of assembly code,  we employed identical prompts across all models to generate outputs. 
\caption{ASMA-Bench (In-the-Wild) experimental results. GPT-4-Turbo responses were collected through three independent query trials to ensure evaluation consistency. Prompts are documented in Appendix B.}
\label{tab:eval:ASMABench}
%\vspace{-4mm}

\end{table*}


==> tables/eval-BCSD_MRR_old.tex <==

\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt} % 增加列间距
\renewcommand{\arraystretch}{1.5} % 增加行高
%\vspace{-2mm}

\begin{tabular}{rcccccccc}
\toprule
          & \multicolumn{8}{c}{\textbf{MRR(Pool size 500)}}                                                                   \\ \cline{2-9} 
\multicolumn{1}{c}{\multirow{0}{*}{\textbf{Models}}} & 
  \multicolumn{1}{c}{Binutils} & 
  \multicolumn{1}{c}{Coreutils} &
  \multicolumn{1}{c}{Curl} &
  \multicolumn{1}{c}{ImageMagick} &
  \multicolumn{1}{c}{SQLite} &
  \multicolumn{1}{c}{OpenSSL} &
  \multicolumn{1}{c}{Putty} &
  \multicolumn{1}{c}{\textbf{Average}} \\ \midrule
GPT-4-Turbo    & 0.190 & 0.175 & 0.191 & 0.162 & 0.169 & 0.232 & 0.174 & 0.185 \\
Qwen2.5-Coder-Instruct-14B          & \textbf{0.227}    & 0.179  & 0.224   & 0.226    & 0.172    & 0.246    & 0.212   & 0.212     \\
Qwen2.5-Coder-Instruct-7B           & 0.155    & 0.106  & 0.119   & 0.135    & 0.091    & 0.147    & 0.119   & 0.124     \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Qwen2.5-Coder-Instruct-AT-7.2B}      & 0.225   & 0.194 & \textbf{0.244}  & 0.245   & \textbf{0.189}  & \textbf{0.268}  & \textbf{0.239}   & \textbf{0.257} \\
DeepSeek-Coder-V2-Lite-Instruct-16B & 0.108    & 0.086  & 0.109   & 0.119    & 0.086    & 0.141    & 0.107   & 0.108     \\
DeepSeek-Coder-Instruct-6.7B        & 0.075    & 0.07  & 0.083   & 0.084    & 0.066    & 0.095    & 0.075    & 0.078     \\
\rowcolor[HTML]{EFEFEF} 
\textbf{DeepSeek-Coder-Instruct-AT-6.9B}     & 0.114 & 0.121 & 0.109  & 0.136  & 0.101   & 0.152 & 0.163 & 0.128  \\
CodeLlama-Instruct-13B              & 0.079    & 0.068  & 0.083   & 0.066    & 0.062    & 0.119    & 0.082   & 0.08     \\
CodeLlama-Instruct-7B               & 0.08       & 0.07  & 0.095   & 0.078     & 0.046    & 0.113    & 0.071    & 0.079     \\
\rowcolor[HTML]{EFEFEF} 
\textbf{CodeLlama-Instruct-AT-7.2B}          & 0.092  & 0.072 & 0.088 & 0.087 & 0.074 & 0.113  & 0.109  & 0.091 \\
Vicuna1.5-13B                       & 0.006    & 0.01  & 0.007   & 0.009    & 0.005    & 0.008    & 0.005   & 0.007     \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Vicuna1.5-AT-13.2B}                  & 0.208      & \textbf{0.258}    & 0.242     & \textbf{0.261}      & 0.158      & 0.2        & 0.202     & 0.218    \\ 
\bottomrule
% \textbf{Average} &
%   \textbf{0.127} &
%   \textbf{0.141} &
%   \textbf{0.129} &
%   \textbf{0.128} &
%   \textbf{0.116} &
%   \textbf{0.136} &
%   \textbf{0.146} &
%   \textbf{ } \\ \bottomrule
\end{tabular}
\caption{BCSD experimental results. Bold number indicates the best performance among all models.}
\label{tab:eval:BCSD:MRR}
%\vspace{-2mm}

\end{table*}

==> tables/token_frequency.tex <==
\begin{table*}[h]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{r|cc}
\toprule
\multicolumn{1}{c|}{\textbf{Models}} & \textbf{Avg. Length} & \textbf{Recall@1 (\%)} \\ 
\midrule
GPT-4-Turbo & 67.49 & 41.45 \\
Qwen2.5-Coder-Instruct-GGUF\textsubscript{14B} & 40.23 & 30.00 \\
DeepSeek-Coder-V2-Lite-Instruct\textsubscript{16B} & 138.50 & 12.98 \\
CodeLlama-Instruct\textsubscript{13B} & 45.63 & 16.10 \\
ASMA-Tune\textsubscript{13B}(Ours) & \cellcolor[HTML]{EFEFEF}42.52 & \cellcolor[HTML]{EFEFEF}50.86 \\ 
\bottomrule
\end{tabular}
\caption{Comparative analysis of response length and recall@1.}
\label{tab:token_frequence}  % 标签应紧接在caption之后
\end{table*}

